Density-optimized Intersection-free Mapping and Matrix Multiplication for Join-Project Operations (extended version)

A Join-Project operation is a join operation followed by a duplicate eliminating projection operation. It is used in a large variety of applications, including entity matching, set analytics, and graph analytics. Previous work proposes a hybrid design that exploits the classical solution (i.e., join and deduplication), and MM (matrix multiplication) to process the sparse and the dense portions of the input data, respectively. However, we observe three problems in the state-of-the-art solution: 1) The outputs of the sparse and dense portions overlap, requiring an extra deduplication step; 2) Its table-to-matrix transformation makes an over-simplified assumption of the attribute values; and 3) There is a mismatch between the employed MM in BLAS packages and the characteristics of the Join-Project operation. In this paper, we propose DIM3, an optimized algorithm for the Join-Project operation. To address 1), we propose an intersection-free partition method to completely remove the final deduplication step. For 2), we develop an optimized design for mapping attribute values to natural numbers. For 3), we propose DenseEC and SparseBMM algorithms to exploit the structure of Join-Project for better efficiency. Moreover, we extend DIM3 to consider partial result caching and support Join-op queries, including Join-Aggregate and MJP (Multi-way Joins with Projection). Experimental results using both real-world and synthetic data sets show that DIM3 outperforms previous Join-Project solutions by a factor of 2.3x-18x. Compared to RDBMSs, DIM3 achieves orders of magnitude speedups.

==> 2previous.tex <==
\section{Previous Solutions} \label{sec:background}

In this section, we classify the algorithms for Join-Project operations in databases and related research into three categories, and then analyze their advantages and disadvantages. Given table $R(x,y)$ and $S(z,y)$, let $|X|$, $|Y|$ and $|Z|$ denote the number of distinct $x$, $y$ and $z$. Taking $|Y|$ for example, it equals to $|\Pi_y(R) \cup \Pi_y(S)|$. 

\textbf{Hash based algorithms.} The most distinct feature of this kind of algorithms is that it divides Join-Project operation into join operation and projection operation (or more precisely, deduplication operation). They are the mainstream algorithms currently used in databases. There are a lot of research and algorithms about join operation \cite{join1992,VLDB09Join,VLDB13Join}, and a reasonable algorithm can be chosen according to factors such as the input size, whether the input is indexed or not, etc. Deduplication operation can be performed by using hash tables \cite{kocberber2013meet} or other indexes \cite{Btree2011,Btree2016,kraska2018case}. We call these algorithms hash based algorithms, because the most representative algorithm of them is to perform hash join first and then use hash table to deduplicate. Since the intermediate results produced by join operation need to be deduplicated one by one, the time complexity of this algorithm is $\Theta(|R|+|S|+|OUT_J|)$. The bottleneck of these algorithms is the deduplication operation: even if there are only a few duplicate intermediate results, the algorithm still needs to deduplicate all the $|OUT_J|$ results, and the $|OUT_J|$ can be very large.

\textbf{Matrix multiplication based algorithms.} The table $R$ and $S$ are transformed into matrix $\mathbf{A}^{x\times y}$ and $\mathbf{B}^{y\times z}$, and then the matrix multiplication operation is performed to get the result matrix $\mathbf{C}^{x\times z}$. In the process of constructing the matrix, the matrix $\mathbf{A}_{i,j}=1$ if and only if tuple $(i,j)\in R$ (similarly for $S$). After finishing the matrix multiplication, each element of matrix $\mathbf{C}^{x\times z}$ is traversed to find all the tuples $(i,j)$ that make $\mathbf{C}_{i,j}>0$. These tuples are the final results of Join-Project operation. Matrix multiplication requires the input to satisfy or approximately satisfy the condition of being consecutive natural numbers starting from 0, otherwise, the transformation from tuples to matrix cannot be performed. Therefore, it faces the extra overhead of mapping the input from original values to consecutive matrix-required values. However, it has the advantage that the result of matrix multiplication can be directly converted to the non-repeated Join-Project result, and the computing process can be accelerated by using many advanced techniques \cite{saule2013performance,dalton2015optimizing,kurzak2009optimizing}.

There are two kinds of specific implementations for matrix multiplication: dense matrix multiplication and sparse matrix multiplication. The time complexity of dense matrix multiplication is $\Theta(|R|+|S|+M(|X|,|Y|,|Z|)+|X||Z|)$, where $M(|X|,|Y|,|Z|)$ is the complexity of computing the matrix multiplication and $|X||Z|$ is the complexity of traversing the result matrix. In \cite{SIGMOD20}, $M(|X|,|Y|,|Z|)$ proved to be equal to $\mathcal{O}(|X||Y||Z|\beta^{\omega-3})$, where $\beta=min(|X|,|Y|,|Z|)$ and $2\le \omega < 3$. In recent research \cite{matrix2018}, it is proved that $omega$ can be equal to 2.373 and possibly smaller. The time complexity of sparse matrix multiplication is $\Theta(|R|+|S|+|OUT_J|)$, and we will discuss this algorithm in detail in the next section.

\textbf{Algorithms that combine hash and matrix multiplication.} These algorithms are mainly based on the observation that hash based algorithms perform better when the data is sparse while matrix multiplication based algorithms perform better when the data is dense. Amossen et al. \cite{ICDT09} proposed an algorithm to partition the data into the dense and sparse part according to degrees of $x$, $y$, and $z$. Then matrix multiplication is performed between the dense parts and the hash based algorithm is performed between the remaining parts. It should be noted that although their paper is titled as sparse matrix multiplication, all of their runtime analyses are based on dense matrix multiplication. Deep et al. \cite{SIGMOD20} corrected some errors in the runtime analyses of \cite{ICDT09} and implemented the algorithm for experimental comparison. They also extend the algorithm to boolean set intersection and many other application scenarios. However, the problems still existing in their algorithm are as follows:
\begin{enumerate}
  \item The result of the dense part and the non-dense part may have duplicated tuples. So, it still needs to perform deduplication when merging the results of the two parts.
  \item The optimal segmentation threshold is difficult to obtain, which requires a lot of statistical information and a large computational overhead.
  \item In order to segment the dataset, the degrees of $x$, $y$ and $z$ are required. The process of counting degrees itself incurs a lot of computational overhead.
\end{enumerate}

With respect to time complexity, Amossen et al. \cite{ICDT09} analyzed and compared the complexity of the hash based algorithms and the two kinds of matrix multiplication algorithms, but their comparison has some flaws. Their comparison is based on the worst case, where the join operation produces the most intermediate results. However, in this case, the time complexity of dense matrix multiplication will be smaller than the $\mathcal{O}(n^{2.376})$ they use, that is, the matrix size will be smaller than $n \times n$. Similarly, their time complexity \cite{TAGL05Spmm} of sparse matrix multiplication makes the same assumption and thus is incorrect. We will show this in detail in Section \ref{sec:complex}.

In addition, \cite{ICDT21Enum} studied enumeration algorithms for conjunctive queries with projection from a theoretical perspective. \cite{PODS20Parallel} studied parallel algorithms for Join-Aggregate queries, including line queries, star queries and tree queries.


==> 6implementation.tex <==
\section{Discussion}

\Paragraph{Implementation in Database Systems} Currently, database systems
divide a Join-Project operation into a join operation and a deduplication
operation, while DIM$^3$ treats them as an integral operation.  To take
advantage of DIM$^3$, the query optimizer needs to traverse the query plan and
combine successive join and deduplication into a single Join-Project operation
so that DIM$^3$ can be applied.
%
Join-Aggregate can be handled similarly.
%
Moreover, the query optimizer can construct Join-Project operations by pushing
the deduplication operation down to certain join operations.  The DP algorithm
in Section~\ref{sec:cq} can be used to optimize the query plan for multi-way
joins with projection.

% 删除 ‘Parallel DIM$^3$’，因为我们已经实现了简单的并行并进行实验比较了。
\Removed{
\Paragraph{Parallel DIM$^3$} DIM$^3$ can be easily parallelized. The mapping
phase, SparseBMM, and DenseEC can all be divided into independent sub-tasks to
be executed by multiple threads.  Specifically, for the mapping phase, each
partition can be processed with a parallel thread.  In fact, the considerations
are similar to hash joins~\cite{VLDB09Join,VLDB13Join}.  For SparseBMM and
DenseEC, disjoint sets of $x$'s (i.e., outer-loop iterations) can be processed
by different threads.  It is possible to employ techniques proposed in the
context of parallelization for matrix
multiplication~\cite{SISC12DCSR,buluc2008challenges,liu2019register}.
}

\Paragraph{Out-of-core Computation} When the input tables or the results are
too large to fit in the allocated memory, we can partition the input tables
according to $R.x$ and $S.z$.  Then, we load each pair of $R.x$ partition and
$S.z$ partition into memory and employ DIM$^3$ to compute the results.
%
An alternative way is to partition the tables according to the join key $y$.
However, in this case, the intermediate results from different partitions may
contain duplicates.  Therefore, a final deduplication step is necessary.


==> 7experimentF.tex <==
  
  % \begin{figure*}[t]
  %   \subfigcapskip=-4pt
  %   \subfigure[$|OUT|$ = 10K, $|OUT_J|$ increases.]{
  %     \includegraphics[width=0.23\linewidth]{fig/ana1-eps-converted-to.pdf}
  %     \label{fig:ana5}
  %   }
  %   \subfigure[$|OUT|$ = 3.6M, $|OUT_J|$ increases.]{
  %     \includegraphics[width=0.23\linewidth]{fig/ana2-eps-converted-to.pdf}
  %     \label{fig:ana6}
  %   }
  %   \subfigure[$|OUT_J|$ = 3.3B, $|OUT|$ decreases.]{
  %     \includegraphics[width=0.23\linewidth]{fig/ana3-eps-converted-to.pdf}
  %     \label{fig:ana7}
  %   }
  %   \subfigure[$|OUT_J|$ = 0.33B, $|OUT|$ decreases.]{
  %     \includegraphics[width=0.23\linewidth]{fig/ana4-eps-converted-to.pdf}
  %     \label{fig:ana8}
  %   }
  %   \vspace{-8pt}
  %   \caption{\textcolor{red}{TODO: remove SparseBMM and DenseEC in this fig. Comparison between DIM3, DHK and Classical.}Evaluation of the abaility of DIM$^3$ to combine its components. (In each set of experiments, we fixed one of $|OUT_J|$ and $|OUT|$ and changed the other to simulate variations of data characteristics, such as density and skew. Skew ratio, x-axis of (c)(d), is calculated by the percentage of data owned by top 10\% of $R.x$ or $S.z$)}
  %   \label{fig:generated2}
  %   \vspace{-12pt}
  % \end{figure*}



==> a1threshold.tex <==
\section{Analysis of DIM$^3$} \label{sec:threshold}

In this section, we compute the three functions used in the DIM$^3$
algorithm to select different evaluation paths.  We verify the
accuracy of our computation using experiments on synthetic data
sets.
%
Then, we analyze the time complexity of DIM$^3$ and compare it with
previous solutions.
%
Table~\ref{tab:symbol} lists the symbols (time constants) used in this
section, which can be measured in advance.

\begin{table}[t]
  \small
  \caption{Symbols used in Section~\ref{sec:threshold}.}
  \label{tab:symbol}
  \vspace{-6pt}
  \begin{tabular}{lp{0.8\columnwidth}}
    \hline
    Symbol & Description \\
    \hline
    %$|R|$ ($|S|$) & The size of input table $R$ ($S$) \\
    %$|OUT_J|$ & The size of intermediate results generated by join \\
    %$|OUT|$ & The size of final Join-Project results \\
    %$|X|$, $|Y|$, $|Z|$ & The number of distinct $x$, $y$ and $z$ \\
    %                    & Taking $|Y|$ for example, it equals to $|\Pi_y(R) \cup \Pi_y(S)|$. \\
    %$m_{x_i}$ ($m_{z_i}$) & The number of $y$ corresponding to $x_i$ ($z_i$), $|\sigma_{x=x_i}R(x,y)|$ ($|\sigma_{z=z_i}S(z,y)|$) \\
    %                      & They can be abbreviated as $m_x$ ($m_z$) when it is clear from the context. \\
    $t_{seqR}$ & time for sequential memory read \\
    $t_{randR}$ & time for random memory read \\
    $t_{randRW}$ & time for random memory read-modify-write\\
    $t_{hash}$ & time of a lookup or insertion to plain hash table \\
    %$t_{map\_L\&I}$ & time of a lookup or insertion to our optimized hash table in mapping phase \\
    $t_{map}$ & time to access the optimized hash table in mapping phase \\
    $t_{ECs}$ & time of a comparison for the non-SIMD method in DenseEC \\
    $t_{ECd}$ & time of a comparison for the SIMD method in DenseEC \\ 
    \hline
\end{tabular}
  \vspace{-0.2in}
\end{table}


\subsection{Strategy Selection ($f_1$)} \label{sec:threshold:alg}

At the beginning of DIM$^3$, we determine whether to use the
classical solution to avoid the mapping overhead with
function $f_1$.

\begin{figure}[h]
  \centering
  \vspace{-10pt}

  \includegraphics[width=\linewidth]{fig/algthreshold-eps-converted-to.pdf}

  \vspace{-10pt}

  \caption{Comparison of three algorithms varying $|OUT_J|$
of joining two tables each having $10^6$ tuples.}

  \vspace{-6pt}

  \label{fig:algthreshold}
\end{figure}

\begin{figure*}[t]
  \centering
  \subfigcapskip=-6pt
  % 移除子标题中的‘Function’，为了省一行
  \subfigure[\Removed{Function} $f_1$ for strategy selection]{
    \includegraphics[width=0.3\linewidth]{fig/threshold1-eps-converted-to.pdf}
    \label{fig:thr:alg}
  }
  \subfigure[\Removed{Function} $f_3$ for selecting bitmap comparison method]{
    \includegraphics[width=0.3\linewidth]{fig/threshold2-eps-converted-to.pdf}
    \label{fig:thr:r}
  }
  \subfigure[\Removed{Function} $f_2$ for deciding column density]{
    \includegraphics[width=0.3\linewidth]{fig/threshold3-eps-converted-to.pdf}
    \label{fig:thr:s}
  }

  \vspace{-6pt}

  \caption{Effectiveness of the three functions for choosing
evaluation paths in DIM$^3$.}

  \vspace{-12pt}
\end{figure*}

Figure~\ref{fig:algthreshold} compares the classical solution,
mapping+SparseBMM, and mapping+DenseEC.  We generate $10^6$ tuples in
tables $R$ and $S$.  The values of columns $x$, $y$, and $z$ are
randomly chosen in [0, $N_{MAX}$], where $N_{MAX}$ ranges from $10^3$
to $10^8$. The data gets more sparse and $|OUT_J|$ becomes smaller as
$N_{MAX}$ increases.  The X-axis shows $|OUT_J|$, while the Y-axis
reports execution time in seconds.  Please note the logarithmic scale.
We see that the classical solution performs the best only when the
data is extremely sparse (i.e., $|OUT_J|$ is very small).  In such
cases, no $S.z$ will be judged as dense and DenseEC will not be used.
Therefore, the hybrid strategy has degenerated into mapping+SparseBMM.

Given this, function $f_1$ only needs to compare the classical
solution with mapping+SparseBMM.  We have the following:
%
\begin{align}
%
&
f_1(|R|,|S|,|OUT_J|)=(T_{mapping}+T_{SparseBMM})-(T_{join}+T_{dedup})
\nonumber\\
%
& = T_{mapping} + (T_{SparseBMM}- T_{join}) - T_{dedup} \nonumber\\
%
& \approx 2(|R|+|S|)t_{map} + |OUT_J|* t_{randRW} - |OUT_J|t_{hash} 
%
\label{for:alg}
%
\end{align}
%
Note that SparseBMM employs CSR and has smaller costs than normal hash
joins as discussed in Section~\ref{sec:bspmm}.  We estimate
$T_{SparseBMM}- T_{join} \approx |OUT_J|* t_{randRW}$.   The
deduplication performs a hash table access for every join output
tuple.  Therefore, its cost is estimated as $|OUT_J|t_{hash}$.  When
$f_1 > 0$, the classical solution is faster and will be chosen in
DIM$^3$.

%When selecting this threshold, we are at line~\ref{alg:main:hash} of Algorithm~\ref{alg:main}. $|R|$, $|S|$ and $|OUT_J|$ are known. Let $T_{mapping}+T_{BSPMM}$ and $T_{join}+T_{dedup}$ represent the costs of SparseBMM with mapping and classical solutions. Recall that in Section~\ref{sec:bspmm} we have analyzed that the time overhead of SparseBMM excluding SPA access should be slightly smaller than hash join, that is
%$$
%T_{BSPMM}- T_{join} \approx |OUT_J|* t_{randRW}
%$$

% I have combined the two different map costs for simplicity
%\begin{align}
%  T_{mapping} = (2|R|+|S|)T_{map\_L\&I}+|S|T_{map\_L} \label{for:Tmapping}
%\end{align}.

\Paragraph{Effectiveness of $f_1$}
%
Figure~\ref{fig:thr:alg} compares the measured running time and the
estimated running time of the classical solution and
mapping+SparseBMM.  In this experiment, we generate random data with
column values in the range of 0 to $10^7$.  We vary $|R|$=$|S|$ from 5
million to 60 million.  The X-axis shows the join result size.  The
Y-axis reports the running time.  From the figure, we see that the
estimated times show consistent trends compared to the measured times.
Function $f_1$ models the intersection of the curves for the two
algorithms.  We see that the intersection points of the measured and
estimated time curves are very close, confirming the effectiveness of
$f_1$ for strategy selection.


\subsection{Bitmap Comparison in DenseEC ($f_3$)} \label{sec:threshold:r}

Line~\ref{alg:ec:R} of the DenseEC Algorithm (Algorithm~\ref{alg:ec})
uses function $f_3$ to determine if the SIMD or non-SIMD method should
be used to compare $Bitmap_x$ and $Bitmap_z$.   

% Although in DIM$^3$ this threshold selection is after the partitioning of table $S$ (Threshold $\theta_2$), we introduce Threshold $\theta_3$ first since the conclusions here are used in Threshold $\theta_2$. 

Let $m_{x=x_i}$=$|\sigma_{x=x_i}R(x,y)|$ and $m_{z=z_j}$ =
$|\sigma_{z=z_j}S(z,y)|$ be the numbers of $y$'s in row $x_i$ and
column $z_j$, respectively.  They can be abbreviated as $m_x$ and
$m_z$ when it is clear from the context.  The two bitmaps have $|Y|$
bits.  $m_x$ ($m_z$) bits in $Bitmap_x$ ($Bitmap_z$) are 1's.  

% This threshold selection matters, because for given $x$ and $z$, the count of comparison in the nonSIMD method does not exceed $m_x$, while that of the SIMD method can reach $\frac{|Y|}{256}$. If the threshold is too small, a large number of bitmaps will be fully traversed and compared. If it is too large, the benefits of SIMD instructions will not be fully exploited.

In the non-SIMD method, the comparison stops as soon as a check hits a
set bit in $Bitmap_z$.  The probability that the check hits a set bit
is $p_s=\frac{m_z}{|Y|}$.  The number of checks follows a geometric
distribution with probability $p_s$, and the method performs at most
$m_x$ checks.  Hence, the expected number of checks is calculated as:
%
\vspace{-0.05in}
$$
%
  \sum_{i=1}^{m_x}i(1-p_s)^{i-1}p_s + m_x(1-p_s)^{m_x} = \tfrac{1-(1-p_s)^{m_x}}{p_s}
%
\vspace{-0.05in}
$$
%

In the SIMD method, every SIMD comparison checks 256 bits in the two
bitmaps.  When the bits at the same position in the two bitmaps are
both set, the comparison returns true and the process stops.  The
probability that an SIMD comparison returns true is
$p_d=1-(1-\frac{m_xm_z}{|Y|^2})^{256}$.  The number of SIMD checks
follows a geometric distribution with probability $p_d$, and the
method performs at most $\frac{|Y|}{256}$ checks. Hence, the expected
number of checks is calculated as
$\tfrac{1-(1-p_d)^{\frac{|Y|}{256}}}{p_d}$.

% It should be clarified that the assumptions for the two estimation models are slightly different. It is assumed that all the tuples of $(z,y)$ are distinct in the nonSIMD method, while it is assumed that all the tuples of both $(x,y)$ and $(z,y)$ are distinct in the SIMD method. Although the accuracy of the estimation decreases when the conditions are not satisfied, it is still acceptable because our goal is to select a potentially faster method with as little cost as possible.

Then, the computed expectations of the two methods can be multiplied
by $t_{ECs}$ and $t_{ECd}$, respectively, to obtain the estimation of
running time.  Thus, we compute $f_3$ as follows.
%
\vspace{-0.05in}
\begin{equation}
%
  f_3(m_x,m_z,|Y|) = \frac{1-(1-\frac{m_z}{|Y|})^{m_x}}{\frac{m_z}{|Y|}}t_{ECs}-\frac{1-(1-\frac{m_xm_z}{|Y|^2})^{|Y|}}{1-(1-\frac{m_xm_z}{|Y|^2})^{256}}t_{ECd}
%
\vspace{-0.05in}
\end{equation}
%
When $f_3 > 0$, the SIMD method is preferred. Otherwise, the non-SIMD method is selected.

\Paragraph{Optimization} Note that $m_x$ and $|Y|$ are constants in
the for-loop at line~\ref{alg:ec:forSz} of Algorithm~\ref{alg:ec}.
$f_3(m_x,m_z,|Y|)$ is monotonically increasing with $m_z$. Therefore,
an optimization is to use binary search to find the threshold value of
$m_{zt}$ so that $f(m_x,m_{zt},|Y|)=0$.  Then, we can select the SIMD
method if $m_z > m_{zt}$.  In this way, many computations can be
avoided.

\Paragraph{Effectiveness of $f_3$}
%
Figure~\ref{fig:thr:r} compares the measured running time and the
estimated running time of the SIMD and non-SIMD methods.  From the
figure, we see that (i) the estimated values are always smaller than
the measured values because some runtime overheads, such as the
for-loop, are not taken into consideration; (ii) the estimated curves
show similar trends as the measured curves; and (iii) the intersection
points of the two sets of curves are very close.  As function $f_3$
models the intersection point, Figure~\ref{fig:thr:r} confirms the
effectiveness of $f_3$.

%A comparison of the actual and estimated running time is shown in Figure~\ref{fig:thr:r}. The estimated value is always smaller than its actual value because some runtime overheads such as \textit{for} loops are not taken into consideration, but the threshold we look for is vary accurate. Besides, it can also be seen that the SIMD method does bring performance improvement when the data gets dense.

\subsection{Dense vs. Sparse Partitions ($f_2$)} \label{sec:threshold:s}

At line~\ref{alg:main:S} in DIM$^3$ (Algorithm~\ref{alg:main}),
intersection-free partitioning uses function $f_2$ to determine if
$S.z$ column is dense or sparse.

% This threshold determines how many $z$ will be assigned to DenseEC and thus is important. If it is too small, the algorithm degrades into SparseBMM and the acceleration for the dense is not significant. If it is too large, the overhead of enumerating and checking too many $<x,z>$ pairs in DenseEC slows down the algorithm.

Suppose we compute $f_2$ for column $z_j$.  The number of join results
with respect to $z_j$ can be estimated as \Removed{$\tfrac{m_{z=z_j}}{|Z|}|OUT_J|$}
\NewlyAdded{$\tfrac{m_{z=z_j}}{|R|}|OUT_J|$}.  
We denote this number as $OUT_{J,z_j}$.

% Let us assume that we are determining the division of $z_1$ at this point. All the $m_x$ and $m_z$ are counted in advance. Therefore, the number of join results with respect to $z_1$ can be calculated by $\sum_{i=1}^{|X|}(m_{x=x_i}*m_{z=z_1})$, denoted as $out\_j_{z_1}$. 

If $f_2$ decides that $z_j$ is sparse, then SparseBMM will process it.
We estimate the cost of SparseBMM for $z_j$ as follows:
%
\vspace{-0.05in} $$
%
\tfrac{(2|X|+|R|)t_{seqR}+2|R|*t_{randR}}{|Z|}+ OUT_{J,z_j}(
t_{seqR}+ t_{randRW})
%
\vspace{-0.05in} $$ 
%
The first component computes the cost of the two for-loops at Line
2--3 amortized to one of $|Z|$ columns.  The second component
estimates the cost of Line 4--7.

If $f_2$ decides that $z_j$ is dense, then DenseEC will process it.
We estimate the overhead for each \revise{$($}$x_i$,$z_j$\revise{$)$} of DenseEC as in
Section~\ref{sec:threshold:r}, which can be summed up to obtain the
cost for processing the entire column $z_j$:
%
\vspace{-0.05in} $$
%
\sum_{i=1}^{|X|}min(\tfrac{1-(1-\tfrac{m_{z_j}}{|Y|})^{m_{x_i}}}{\tfrac{m_{z_j}}{|Y|}}t_{ECs},\tfrac{1-(1-\tfrac{m_{x_i}m_{z_j}}{|Y|^2})^{|Y|}}{1-(1-\tfrac{m_{x_i}m_{z_j}}{|Y|^2})^{256}}t_{ECd})
%
\vspace{-0.05in} $$
%
This formula can be costly to compute because it may sum over up to
$|X|$ values.  To reduce the computation cost, we approximate the
computation as follows.  We group $m_x$ according to the value of
$\lfloor\lg(m_x)\rfloor*10+\lfloor\frac{m_x}{10^{\lfloor\lg(m_x)\rfloor}}\rfloor$.
Then we represent each group by the median of the group in the
calculation.
%
Similarly, we divide $m_z$ into 100 groups according to
$\frac{|Y|}{100}$ and use the median of each group.  In this way, we
avoid the calculation of many similar values.

Finally, $f_2$ is computed as the difference between the above two
computed costs.


\Paragraph{Effectiveness of $f_2$}
%
Figure~\ref{fig:thr:s} compares the measured running time and the
estimated running time of SparseBMM and DenseEC.  From the figure, we
see that (i) the estimated curves show similar trends as the measured
curves; and (ii) the intersection points of the two sets of curves are
close.  This demonstrates the effectiveness of using function $f_2$
for intersection-free partitioning.

%The test of the accuracy of this threshold selection method is shown in Figure~\ref{fig:thr:s}. It can be observed that the trend of our estimated time curve is consistent with its actual curve, and the chosen threshold is very close to the optimal threshold. The only drawback is that the estimated \textit{Dense} curve deviates from its actual curve when the data density is small, because there are many trivial overheads such as allocating bitmap memory are not taken into consideration.

\subsection{Complexity of DIM$^3$} \label{sec:complex}

%it is clear that the time complexity of DIM$^3$ is determined by the distribution of the input data and our threshold selection methods.  Assume that all thresholds are chosen relatively accurately. The time complexity can be expressed as 

Based on the analysis in
Section~\ref{sec:threshold:alg}--~\ref{sec:threshold:s}, the time
complexity of DIM$^3$ can be expressed as the following:
%
\begin{align} & Complexity_{DIM^3} = \mathcal{O}(|R|+|S|+ \nonumber\\
&\sum_{j=1}^{|Z|} min( OUT_{J,z_j}, \sum_{i=1}^{|X|}min(
\tfrac{1-(1-\tfrac{m_{z_j}}{|Y|})^{m_{x_i}}}{\tfrac{m_{z_j}}{|Y|}},
\tfrac{1-(1-\tfrac{m_{x_i}m_{z_i}}{|Y|^2})^{|Y|}}{1-(1-\tfrac{m_{x_i}m_{z_j}}{|Y|^2})^{256}})))
\label{for:time} \end{align}
%
Thus, we have the following:
%
\vspace{-0.05in} $$
%
Complexity_{DIM^3} \leq
\mathcal{O}(|R|+|S|+\sum_{i=1}^{|Z|}out\_j_{z_i}) =
\mathcal{O}(|R|+|S|+|OUT_J|) \nonumber
%
\vspace{-0.05in}
%
$$ Recall that $\mathcal{O}(|R|+|S|+|OUT_J|)$ is the time complexity
of the classical solution and SparseBMM.  The above inequality shows
that the complexity of DIM$^3$ is no greater than that of the
classical solutions and the SparseBMM.
%
This is a natural result since SparseBMM is a component of DIM$^3$. 

Next, we compare DIM$^3$ and the dense MM.  We assume that
$|X|=|Y|=|Z|=n$ and $\frac{m_{x_i}}{|Y|}=\alpha,
\frac{m{z_j}}{|Y|}=\beta$ for all $x_i$ and $z_j$. That is, the data
are uniformly distributed in the $n \times n$ matrices. From
formula~\ref{for:time}, we get
%
\begin{align} 
%
& Complexity_{DIM^3}  =  \mathcal{O}(|R|+|S|+ \nonumber\\ & n^2
min(\tfrac{|OUT_J|}{n^2}, \frac{1-(1-\beta)^{\alpha
n}}{\beta},\frac{1-(1-\alpha\beta)^n}{1-(1-\alpha\beta)^{256}}))
\nonumber
%
\end{align}
%
Note that the three components in $min$ represent the time complexity
of SparseBMM, non-SIMD and SIMD methods in DenseEC, respectively.
According to \cite{matrix2018}, the time complexity of dense MM is
$\mathcal{O}(|R|+|S|+n^{2.373})$.  We can remove $|R|+|S|+n^2$ from
both formulas.  Hence, we need to compare the three components in
$min$ with $n^{0.373}$ under different situations.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.8\linewidth]{fig/complexity2-eps-converted-to.pdf}
  \vspace{-8pt}
  \caption{Comparison of the time complexity between DIM$^3$ and dense
MM.}
  \label{fig:complex}
  \vspace{-10pt}

\end{figure}

Figure~\ref{fig:complex} compares these four polynomials under
different $\alpha$, $\beta$ and $n$.  The color of a point represents
the polynomial that gives the smallest value for given parameters.
From the figure, we see that the dense MM does not show up in any
cases.  This means that DIM$^3$ is better than dense MM in all the
parameter combinations in terms of time complexity.

%there is no case where dense MM is the smallest expression, demonstrating the superiority of DIM$^3$ in terms of time complexity. Additionally, the yellow regions occupy the majority of the area, demonstrating that DenseEC does lead to significant performance gains in many situations.

However, it should be noted that there is a gap between the
theoretical time complexity and the measured running time.  The
constant factor is different for each algorithm. Therefore, although
the yellow area where the SIMD DenseEC is used is quite large, it may
not be the case for the actual running time.  Hence, function $f_1$,
$f_2$, and $f_3$ are used to select the good evaluation paths in the
algorithm.

\Paragraph{Problem in Analysis of Previous Study}  We find that there
are problems in the analysis in the previous study~\cite{ICDT09}.  It
compares the time complexity of the classical solution and the dense
MM.  It assumes that the input size $|R|$=$|S|$=$N$, the dimension of
the matrices $|X|$=$|Y|$=$|Z_{column}|$=$n$, and the output size
$|OUT|$=$Z$.  (Note that $Z$ is used differently in this previous
work.)
%
In the worst case, it assumes that the join can produce
$N\sqrt{Z}$ results, while the final result size after
deduplication is $Z$.  Hence, the classical solution takes
$\mathcal{O}(N\sqrt{Z})$ time.  For the dense MM, the time complexity
of multiplying two $n \times n$ matrices is computed as
$\mathcal{O}(n^{2.376})$~\cite{matrix1987}.  Then, the work considers
the design space while varying $|N|$ and $|Z|$, then depicts the best
algorithm for each design point.  It shows that the classical solution
wins in certain area in the design space.

However, this actually contradicts with common intuition.  In the
worst case, the matrices are dense.  Therefore, the dense MM should be
faster than the classical solution for the dense cases.  In the
following, we prove that this is indeed the case, and the analysis in
the previous work is not correct.

In fact, to achieve the worst case, the dimensions of the two matrices
$\mathbf{R}$ and $\mathbf{S}$ must be $\sqrt{Z} \times
\tfrac{N}{\sqrt{Z}}$ and $\tfrac{N}{\sqrt{Z}} \times \sqrt{Z}$.  Only
when $N$ = $Z$ = $n^2$ can the matrices be square.  For other $N$ and
$Z$ in the design space, the matrix dimensions are different.

In the worst case, there are $\sqrt{Z}$ values in the $x$ column,
$\tfrac{N}{\sqrt{Z}}$ values in the $y$ column, and $\sqrt{Z}$ values
in the $z$ column.  To get the $N\sqrt{Z}$ join result tuples, all the
$x$ values must be connected to all the $y$ values, and all the $y$
values must be connected to all the $z$ values (in the graph view of
the tables).

The complexity of dense MM is
$\mathcal{O}(|X||Y||Z_{column}|\beta^{\omega-3})$, where
$\beta=min(|X|,|Y|,|Z_{column}|)$ and $\omega$ is
2.373~\cite{matrix2018}.  Therefore, plugging in the dimensions of the
worst case, this complexity is 
%
\vspace{-0.05in} $$
%
Complexity_{MM}=\mathcal{O}(N\sqrt{Z}min(\sqrt{Z},
\frac{N}{\sqrt{Z}})^{-0.627})
%
\vspace{-0.05in} $$  
%
Given $Z \leq N^2$, we can see that $min(\sqrt{Z}, \frac{N}{\sqrt{Z}})
\geq 1$.  Thus, we have the following.
%
\vspace{-0.05in} $$
%
Complexity_{MM} \leq \mathcal{O}(N\sqrt{Z}) = Complexity_{classical}
%
\vspace{-0.05in} $$  
%
That is, the dense MM is always better than the classical solution in
the worst case.


%It is obvious that for any $N$ and $Z$ its time complexity is smaller than that of classical solutions. In fact, the time complexity of dense MM in this case is not worse than that of the algorithm proposed by themselves, $\mathcal{O}(N^{0.83}Z^{0.589}+NZ^{0.41})$~\cite{SIGMOD20}. It is also worth mentioning that, in this case, since $m_{z_i}=m_{x_j}=|Y|$ for all $z_i$ and $x_j$ and $|X|=|Z|=\sqrt{Z}$, the time complexity of DIM$^3$ is $\Theta (N+Z)$, which is optimal among all kinds of algorithms.


